Targeted Testing of Compiler Optimizations via Grammar-Level Composition Styles

Ensuring the correctness of compiler optimizations is critical, but existing fuzzers struggle to test optimizations effectively. First, most fuzzers use optimization pipelines (heuristics-based, fixed sequences of passes) as their harness. The phase-ordering problem can enable or preempt transformations, so pipelines inevitably miss optimization interactions; moreover, many optimizations are not scheduled, even at aggressive levels. Second, optimizations typically fire only when inputs satisfy specific structural relationships, which existing generators and mutations struggle to produce. We propose targeted fuzzing of individual optimizations to complement pipeline-based testing. Our key idea is to exploit composition styles - structural relations over program constructs (adjacency, nesting, repetition, ordering) - that optimizations look for. We build a general-purpose, grammar-based mutational fuzzer, TargetFuzz, that (i) mines composition styles from an optimization-relevant corpus, then (ii) rebuilds them inside different contexts offered by a larger, generic corpus via synthesized mutations to test variations of optimization logic. TargetFuzz is adaptable to a new programming language by lightweight, grammar-based, construct annotations - and it automatically synthesizes mutators and crossovers to rebuild composition styles. No need for hand-coded generators or language-specific mutators, which is particularly useful for modular frameworks such as MLIR, whose dialect-based, rapidly evolving ecosystem makes optimizations difficult to fuzz. Our evaluation on LLVM and MLIR shows that TargetFuzz improves coverage by 8% and 11% and triggers optimizations 2.8$\times$ and 2.6$\times$, compared to baseline fuzzers under the targeted fuzzing mode. We show that targeted fuzzing is complementary: it effectively tests all 37 sampled LLVM optimizations, while pipeline-fuzzing missed 12.

==> Figs/approach/mutator_symbols.tex <==
\[
m : \langle \textsf{Cousins}, \langle L_1,\;L_2 \rangle,\,F\,, p\{k=0,d=0\}\rangle
\]

\[
\text{Partial}(m) = n'_{\text{ctx}}:
\]

\[
F \mapsto F', L_1 \mapsto L_1',L_2 \mapsto \ell\]

$$\textsc{Uses}=\{\texttt{sum1}\}$$

==> Figs/approach/mutators_example.tex <==
% ===========================
% Example 1: Loop Fusion via Cousins + Replicate (one-column, simple minipage)
% ===========================
\begin{figure}[t]
\centering

\begin{minipage}[t]{0.32\linewidth}
\raggedright\textbf{Donor + match (\textsf{Cousins})}\par\vspace{0.3em}
\begin{lstlisting}[style=CStyle,
  moredelim=**[is][\bfseries\color{red!70!black}]{<<}{>>},
  moredelim=**[is][\bfseries\color{blue!70!black}]{<a>}{</a>},
  moredelim=**[is][\bfseries\color{teal!70!black}]{<ins>}{</ins>}
]
// Two cousin loops (same ancestor Function)
void F() {
  <<for (int i=0; i<N; ++i) { <a>sum += a[i];</a> }>>
  <<for (int i=0; i<N; ++i) { <a>prod *= b[i];</a> }>>
}
\end{lstlisting}
\end{minipage}\hfill
\begin{minipage}[t]{0.32\linewidth}
\raggedright\textbf{Recipient (before)}\par\vspace{0.3em}
\begin{lstlisting}[style=CStyle,
  moredelim=**[is][\bfseries\color{red!70!black}]{<<}{>>},
  moredelim=**[is][\bfseries\color{blue!70!black}]{<a>}{</a>},
  moredelim=**[is][\bfseries\color{teal!70!black}]{<ins>}{</ins>}
]
void Fp() {
  for (int i=0; i<N; ++i) { <a>sum += a[i];</a> }
  <ins>/* locus ℓ for missing cousin loop */</ins>
}
\end{lstlisting}
\end{minipage}\hfill
\begin{minipage}[t]{0.32\linewidth}
\raggedright\textbf{Recipient (after) — \circled{R} Replicate}\par\vspace{0.3em}
\begin{lstlisting}[style=CStyle,
  moredelim=**[is][\bfseries\color{red!70!black}]{<<}{>>},
  moredelim=**[is][\bfseries\color{blue!70!black}]{<a>}{</a>},
  moredelim=**[is][\bfseries\color{teal!70!black}]{<ins>}{</ins>}
]
void Fp() {
  for (int i=0; i<N; ++i) { <a>sum += a[i];</a> }
  // Replicate: clone anchor into ℓ to re-create cousins
  <<for (int i=0; i<N; ++i) { <a>prod *= b[i];</a> }>>  // inserted at ℓ
}
\end{lstlisting}
\end{minipage}

\caption{End-to-end realization of \textsf{Cousins} via \circled{R} Replicate to enable loop fusion opportunities.}
\label{fig:cousins-replicate}
\vspace{-0.4em}
\end{figure}


==> Program/combined_algs.tex <==
\begin{figure}
\begin{minipage}[t]{0.47\textwidth}
\begin{algorithm}[H]
\caption{Replicate: mutation} 
\label{alg:replicate} 
\begin{algorithmic}[1]
\scriptsize
\Require
    \item[]
        \begin{itemize}[leftmargin=2em]
            \item $ptn \gets$ the composition
            \item $nodes, cxt \gets$ donor's constructs \& context
            \item $params \gets$ composition's hyperparameters
            \item $T \gets$ recipient's parse tree to mutate
        \end{itemize}
\Ensure
    \item[]
        \begin{itemize}[leftmargin=1.5em]
            \item $T_{new} \gets T$ mutated
        \end{itemize}

\State $n_{rm} \gets \text{random.choice}(nodes)$

\State $cxt', n_a \gets \text{Partialize}(pat, cxt, n_{rm})$

\State $cxt_T, n_T, loc \gets \text{MatchContext}(T, cxt', n_a, n_{rm})$
\If{IllegalContext$(cxt_T, params)$}
    \State \textbf{return}
\EndIf
\State $T_{new} \gets \text{Insert}(\text{copy}(n_T), loc)$
\State $\textbf{yield}  T_{new}$

    
\end{algorithmic}
\end{algorithm}
\end{minipage}

\hfill
\begin{minipage}[t]{0.47\textwidth}
\begin{algorithm}[H]
\caption{MatchContext} 
\label{alg:contextmatch} 
\begin{algorithmic}[1]
\scriptsize
\Require
    \item[]
        \begin{itemize}[leftmargin=1.2em]
            \item $T \gets$ recipient's parse tree to mutate
            \item $cxt \gets$ donor's context tree
            \item $[nodes] \gets$ donor's constructs
            \item $n_a, n_{rm} \gets$ donor's anchor \& removed node
            
        \end{itemize}
\Ensure
    \item[]
        \begin{itemize}[leftmargin=1.2em]
            \item $cxt_T \gets $ recipient's context matched
            \item $n_T, loc \gets$ recipient nodes matching $n_a, n_{rm}$
        \end{itemize}

\State $[cxt_{T}] \gets \text{Traverse}(T)$

\For{$cxt_{T} \gets [cxt_{T}]$}

    \If{$cxt_{T}.type == cxt.type$}
        
        \State $n2nodes_T \gets \text{CandidateNodes}(cxt_{T}, [nodes])$
        
        \State $cxt_{T}.sim \gets 0$
        
        \For{$n \gets [nodes]$}
        
            \State $[nodes_{c}] \gets n2nodes_T[n]$

                \State $n_T, s \gets \text{FindHighKLRScore}(n, [nodes_{c}])$

                \State $cxt_{T}.sim \gets sim + s$, 
                
                \State $cxt_{T}.match[n] \gets n_T$
        \EndFor
    \EndIf
\EndFor
\State $cxt_T, match \gets \text{BestContextInT}([cxt_{T}])$

\State \textbf{yield} $cxt_T, match[n_a], match[n_{rm}]$
    
\end{algorithmic}
\end{algorithm}

\end{minipage}
\vspace{-1em}
\end{figure}

==> Program/matchcontext.tex <==
\begin{algorithm}[ht]
\caption{$MatchContext$: Context Matching} 
\label{alg:contextmatch} 
\begin{algorithmic}[1]
\small
\Require
    \item[]
        \begin{itemize}
            \item $T \gets$ the target parse tree to mutate
            \item $cxt \gets$ the donor context tree
            \item $[nodes] \gets$ the donor constructs
            \item $n_a, n_{rm} \gets$ the donor's anchor node \& removed node
            
        \end{itemize}
\Ensure
    \item[]
        \begin{itemize}
        \item $cxt_T \gets $ the target context matched
        \item $n_T, loc_{missing} \gets$ the
        \end{itemize}

$[cxt_{cndt}] \gets \text{traverse}(T)$
\For{$cxt_{cndt} \gets [cxt_{cndt}]$}

    \IF{$cxt_{cndt}.type == cxt.type$}
        \State $trees \gets \text{traverse}(cndt_{cxt})$
        
        \State $n2nodes_T \gets \text{FindCndtNodes}(cxt_{cndt}, [nodes])$
        
        \State $cxt_{cndt}.sim \gets 0$
        
        \FOR{$n$ \gets $[nodes]$}
        
            \STATE $[nodes_{cndt}] \gets n2nodes_T[n]$

                \STATE $n_T, s \gets \text{FindHighKLRScore}(n, [nodes_{cndt}])$

                \STATE $cxt_{cndt}.sim \gets sim + s$, 
                
                \STATE $cxt_{cndt}.match[n] \gets n_T$
    \EndIf
\STATE $cxt_T, match \gets \text{BestCndtContext}([cxt_{cndt}])$

\STATE \textbf{yield} $cxt_T, match[n_a], match[n_{rm}]$
    
\end{algorithmic}
\end{algorithm}



==> Program/replicate.tex <==
\begin{algorithm}[ht]
\caption{$Replicate$: mutation} 
\label{alg:replicate} 
\begin{algorithmic}[1]
\small
\Require
    \item[]
        \begin{itemize}
            \item $ptn \gets$ the pattern
            \item $nodes, cxt \gets$ the donor constructs \& context
            \item $params \gets$ pattern's hyperparameters
            \item $T \gets$ the target parse tree to mutate
        \end{itemize}
\Ensure
    \item[]
        \begin{itemize}
            \item $T_{new} \gets T$ mutated
        \end{itemize}

\State $cxt', n_a, n_{rm} \gets \Partialize(pat, cxt, nodes)$

\State $cxt_T, n_T, loc_{missing} \gets \MatchContext(T, cxt', n_a, n_{rm})$
\IF{IllegalContext$(cxt_T, params)$}
    \State return

\State $T_{new} \gets \Insert(copy(n_T), loc_{missing})$\\

    
\end{algorithmic}
\end{algorithm}


==> Table/approach/mutators.tex <==

\begin{table}[tb]
    \small
    \centering
    \begin{tabularx}{\columnwidth}{p{2cm}|p{3.5cm}|X}
        \header{Mutations} & \header{Composition} & \header{e.g. \textit{Composition-specific mutators}} \\ \toprule
        \circled{R} \textbf{Replicate} 
        & For Loops $L_1, L_2$ are cousins in (context) Function $F$ 
        & In $P$, locate function $F'$ that is similar to $F$ and contains a For Loop $L_1'$ by context matching; replicate $L_1'$ to $L_2'$, make $L_1', L_2'$ cousins \\ \hline
        \circled{M} \textbf{Move} 
        & Arithmetic Expression $E_1, E_2$ are balanced in (context) If-Else $I$
        & In $P$, locate If-Else $I'$ that is similar to $I$ by context matching. If the Arithmetic Expression $E_1'$ exists in one branch of $I'$ and is structurally similar to $E_1$, move another arithmetic expression $E_2'$ in the tree to a location in the other branch. \\ \hline
        \circled{I} \textbf{Insert} 
        & Function Call $F$ exists in (context) Loop $L$ 
        & In $P$, locate Loop $L'$ that is similar to $L$; reparameterize $F$ into $F'$ and insert it at a structurally similar location in $L'$. \\ \hline
        \circled{P} \textbf{Replace} 
        & Arithmetic (e.g., a magic float number $N$) exists in Vector (Array) $V$ 
        & In $P$, locate Vector (Array) $V'$ and its descendant Arithmetic $N'$; reparameterize $N$ and replace $N'$. \\ \hline
    \end{tabularx}
    \vspace{1ex}
    \caption{\tool{} automatically instantiates composition-specific mutators for different constructs.}
    \label{tab:mut_strategy}
    \vspace{-1.5em}
\end{table}


==> Table/eval/coverage.tex <==
\begin{table}[H]
\centering
\caption{Aggregate Line and Branch Coverage on \llvmnumoptim\, LLVM optimizations}
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
  \hline
  \textbf{Fuzzer} & \multicolumn{2}{c|}{\textbf{Target Corpus}} & \multicolumn{2}{c|}{\textbf{Grammarinator}} & \multicolumn{2}{c|}{\textbf{GrayC}} & \multicolumn{2}{c|}{\textbf{SynthFuzz}} & \multicolumn{2}{c|}{\textbf{\tool{}}} \\
  \hline
  & Line & Branch & Line & Branch & Line & Branch & Line & Branch & Line & Branch \\
  Coverage &5881&	2607&	6139&	2891&	5228&	2332&	6930&	3252&	6559&	3093\\
  \hline
\end{tabular}
}
\label{tab:llvm_coverage}
\end{table}
\vspace{-.5em}

\begin{table}[H]
\centering
\caption{Aggregate Line and Branch Coverage on \mlirnumoptim\, MLIR optimizations}
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
  \hline
  \textbf{Fuzzer} & \multicolumn{2}{c|}{\textbf{Target Corpus}} & \multicolumn{2}{c|}{\textbf{Grammarinator}} & \multicolumn{2}{c|}{\textbf{MLIRSmith}} & \multicolumn{2}{c|}{\textbf{SynthFuzz}} & \multicolumn{2}{c|}{\textbf{\tool{}}} \\
  \hline
  & Line & Branch & Line & Branch & Line & Branch & Line & Branch & Line & Branch \\
  Coverage & 1220	&268 &	473 &	60	&331 &	23	&1644&	442&	1223	&307 \\
  \hline
\end{tabular}
}
\label{tab:mlir_coverage}
\vspace{-1em}
\end{table}


==> Text/implementation.tex <==
\section{Implementation}



==> Text/threats.tex <==

\section{Threats to validity}

\textbf{Methodology of collecting optimization corpus.} Encouraged by success stories of generating target-specific tests cases using Large Language Models \cite{xia2024fuzz4all} \cite{lemieux2023codamosa}, we collected out optimization corpus by prompting GPT4o-mini. While all the evaluated fuzzers are tested equally with the same optimization corpus, choosing a different source, e.g., unit tests, a different LLM, or different way of prompting, may produce different results.
